GVE-Leiden: Fast Leiden Algorithm for Community Detection in Shared Memory Setting

Community detection is the problem of identifying natural divisions in networks. Efficient parallel algorithms for identifying such divisions is critical in a number of applications, where the size of datasets have reached significant scales. This technical report presents one of the most efficient implementations of the Leiden algorithm, a high quality community detection method. On a server equipped with dual 16-core Intel Xeon Gold 6226R processors, our Leiden implementation, which we term as GVE-Leiden, outperforms the original Leiden, igraph Leiden, NetworKit Leiden, and cuGraph Leiden (running on NVIDIA A100 GPU) by 436x, 104x, 8.2x, and 3.0x respectively - achieving a processing rate of 403M edges/s on a 3.8B edge graph. In addition, GVE-Leiden improves performance at an average rate of 1.6x for every doubling of threads.

==> src/fig-leiden-hashtable.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:leiden-hashtable--all}
    \includegraphics[width=0.88\linewidth]{out/leiden-hashtable.pdf}
  } \\[-2ex]
  \caption{Illustration of collision-free per-thread hashtables that are well separated in their memory addresses (Far-KV), for two threads. Each hashtable consists of a keys vector, values vector (of size $|V|$), and a key count ($N_0$/$N_1$). The value associated with each key is stored/accumulated in the index pointed by the key. As the key count of each hashtable is updated independently, we allocate it separately on the heap to avoid false cache sharing. These are used in the local-moving and aggregation phases of our Leiden implementation.}
  \label{fig:leiden-hashtable}
\end{figure}


==> src/fig-leiden-pruning.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:leiden-pruning--all}
    \includegraphics[width=0.78\linewidth]{out/leiden-pruning.pdf}
  } \\[-2ex]
  \caption{Illustration of vertex pruning optimization: After processing vertex $1$, it's unmarked. If vertex $1$ changes its community, its neighbors are marked for processing. Community membership of each vertex is depicted by border color, and marked vertices are highlighted in yellow.}
  \label{fig:leiden-pruning}
\end{figure}


==> src/fig-leiden-speedup.tex <==
\begin{figure*}[hbtp]
  \centering
  \subfigure{
    \label{fig:leiden-speedup--all}
    \includegraphics[width=0.98\linewidth]{out/leiden-speedup.pdf}
  } \\[-2ex]
  \caption{Speedup of \textit{GVE-Leiden} with respect to \textit{Vite}, \textit{Grappolo}, and \textit{NetworKit} for each graph in the dataset.}
  \label{fig:leiden-speedup}
\end{figure*}

